Learning Hierarchical Representations of Electronic Health Records for Clinical Outcome Prediction

Clinical outcome prediction based on the Electronic Health Record (EHR) plays a crucial role in improving the quality of healthcare. Conventional deep sequential models fail to capture the rich temporal patterns encoded in the longand irregular clinical event sequences. We make the observation that clinical events at a long time scale exhibit strongtemporal patterns, while events within a short time period tend to be disordered co-occurrence. We thus propose differentiated mechanisms to model clinical events at different time scales. Our model learns hierarchical representationsof event sequences, to adaptively distinguish between short-range and long-range events, and accurately capture coretemporal dependencies. Experimental results on real clinical data show that our model greatly improves over previous state-of-the-art models, achieving AUC scores of 0.94 and 0.90 for predicting death and ICU admission respectively, Our model also successfully identifies important events for different clinical outcome prediction tasks

==> resources/discussion.tex <==
%\subsection{Discussion}



%In order to see if the learned embeddings of heterogeneous events are meaningful, we use LargeVIS~\autocite{tang2016visualizing} to get the 2D projection of all the heterogeneous events. 
%Notice that the same type of events with different attributes have distinct embedding vectors and will be plot in different positions in the pictures in Figure \ref{fig:embedding}.

\subsection{Case Study of Hierarchical Attention Mechanisms}
\begin{figure}[!ht]
\centering
\includegraphics[width=.9\linewidth]{resources/case.png}
\vspace{-.4cm}
\caption{Visualization of the event and temporal attention  }
\vspace{0.0cm}
\label{fig:temporal}
\end{figure}

To help experts to get some clinical insights by our hierarchical model, we visualize  the event attention and temporal attention mechanisms in Figure \ref{fig:temporal}.

From the colored frequency distribution histograms, we can see that irregular event sequences are adaptively segmented into groups. And we can see that some important events are picked out by the event attention score in the groups with high temporal attention scores. Taking the patient B as an example, although the events with the highest attention score of 19th and 24th group are lab tests for potassium and phenytoin with both normal results, resulting in the decreases of prediction score for death, the low temporal attention scores of these two groups indicate that these event groups will not influence the overall prediction result for the patient. Besides, we can see that there are many important events, such as unresponsive conscious level records and the drug input of levophed, in the event groups with high temporal attention score, which infers that the status of the patient is not well. So the final prediction of the model for the patient is death in hospital just as the truth. The subsequence consisting of critical events in the original long event sequence, captured by the hierarchical representations of clinical sequence, may provide long-range clinical insights for medical experts to evaluate the danger level and predict clinical endpoints of patients.

\subsection{Feature Analysis}
Important events for clinical prediction tasks can be picked out by the event attention mechanism in the hierarchical model.  The same events will get different event attention scores due to the local dependency with their surrounding events and the long-term dependency resulting from their phase in the temporal structure.  We divided the samples in each dataset into two groups according to the label to discover some differences of the statistics of the events between patients with different clinical endpoints. Thus, we calculated some statistics, including  the average event attention score,  the 1st quartile, the median, the 3rd quartile, the maximum of attention score and so on, of all kinds of events in each group. The top 10 events in each group  with highest median attention score and 3rd Quartile are listed in Table \ref{tab:top event}(for death prediction task) and Table \ref{tab:top event}(for ICU prediction task) respectively.  As the results, the top events in each group are similar both in term of median and the 1st quartile, indicating that these statistics can represent the distribution of attention score of critical events. We can find that important events in different dataset are different, which indicates that our model are able to capture critical information for different end point prediction tasks. 

\input{table_top_event}






